Evaluation of Local Explanation Methods for Multivariate Time Series Forecasting

Being able to interpret a machine learning model is a crucial task in many applications of machine learning. Specifically, local interpretability is important in determining why a model makes particular predictions. Despite the recent focus on AI interpretability, there has been a lack of research in local interpretability methods for time series forecasting while the few interpretable methods that exist mainly focus on time series classification tasks. In this study, we propose two novel evaluation metrics for time series forecasting: Area Over the Perturbation Curve for Regression and Ablation Percentage Threshold. These two metrics can measure the local fidelity of local explanation models. We extend the theoretical foundation to collect experimental results on two popular datasets, \textit{Rossmann sales} and \textit{electricity}. Both metrics enable a comprehensive comparison of numerous local explanation models and find which metrics are more sensitive. Lastly, we provide heuristical reasoning for this analysis.

==> tables/electricity.tex <==
\newcommand{\mcps}{\multicolumn{1}{p{0.8cm}|}}
\newcommand{\cnt}{\centering}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
                  & \multicolumn{6}{c|}{AOPCR}                                                                                                              & \multicolumn{6}{c|}{APT}                                                                                                                  \\ \hline
Model             & \multicolumn{2}{c|}{TDNN}                     & \multicolumn{2}{c|}{LSTM}                     & \multicolumn{2}{c|}{GBR}                      & \multicolumn{2}{c|}{TDNN}                     & \multicolumn{2}{c|}{LSTM}                     & \multicolumn{2}{c|}{GBR}                      \\ \hline
& \mcps{\cnt positive} & \mcps{\cnt negative}        & \mcps{\cnt positive} & \mcps{\cnt negative}     & \mcps{\cnt positive} & \mcps{\cnt negative}     & \mcps{\cnt positive} & \mcps{\cnt negative}     & \mcps{\cnt positive} & \mcps{\cnt negative}     & \mcps{\cnt positive} & \mcps{\cnt negative}                 \\ \hline
Random &            -0.00050 & -0.00035                     & 0.00000 & -0.00014                    & 0.00008 & -0.00003                    & 0.991 & 0.800                     & 0.523 & 0.508                     & 0.725 & 0.655  \\ \hline
Omission (Global) & \textbf{0.00263} & \textbf{-0.00573}  & 0.08568 & -0.13806                      & 0.06307 & -0.05938                    & 0.883 & 0.682                     & \textbf{0.130} & \textbf{0.114}  & 0.477 & 0.493  \\ \hline
Omission (Local) & 0.00243 & -0.00527                       & 0.06884 & -0.07899                    & 0.04892 & -0.04395                    & 0.900 & 0.707                     & 0.132 & 0.177                     & 0.524 & 0.532  \\ \hline
SHAP &              0.00055 & -0.00430                      & \textbf{0.11379} & \textbf{-0.14165}  & \textbf{0.07067} & \textbf{-0.06664}  & \textbf{0.642} & \textbf{0.363}  & 0.141 & 0.130                      & \textbf{0.348} & \textbf{0.423}  \\ \hline
\end{tabular}


==> tables/rossmann.tex <==
\newcommand{\mcps}{\multicolumn{1}{p{0.8cm}|}}
\newcommand{\cnt}{\centering}

\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
& \multicolumn{6}{c|}{AOPCR} & \multicolumn{6}{c|}{APT}\\ 
\hline
Model             & \multicolumn{2}{c|}{TDNN}                     & \multicolumn{2}{c|}{LSTM}                     & \multicolumn{2}{c|}{GBR}                      & \multicolumn{2}{c|}{TDNN}                     & \multicolumn{2}{c|}{LSTM}                     & \multicolumn{2}{c|}{GBR}                      \\ \hline
& \mcps{\cnt positive} & \mcps{\cnt negative}        & \mcps{\cnt positive} & \mcps{\cnt negative}     & \mcps{\cnt positive} & \mcps{\cnt negative}     & \mcps{\cnt positive} & \mcps{\cnt negative}     & \mcps{\cnt positive} & \mcps{\cnt negative}     & \mcps{\cnt positive} & \mcps{\cnt negative}                 \\ \hline
Random          & 0.00011 & -0.00014                    & 0.00003 & -0.00019                    & -0.00090 & -0.00129                   & 0.842 & 0.908                 & 0.362 & 0.460                     & 0.611 & 0.600  \\ \hline
Omission (Global) & 0.00344 & -0.00279                  & 0.08478 & -0.09673                    & 0.06600 & -0.09787                    & 0.810 & 0.890                 & \textbf{0.093} & \textbf{0.204}  & 0.232 & 0.369  \\ \hline
Omission (Local) & 0.00150 & -0.00126                   & 0.07034 & -0.08011                    & 0.06071 & -0.09026                    & 0.813 & 0.893                 & 0.160 & 0.273                     & 0.263 & 0.393  \\ \hline
SHAP            & \textbf{0.03734} & \textbf{-0.02971}  & \textbf{0.09522} & \textbf{-0.09802}  & \textbf{0.07862} & \textbf{-0.11273}  & \textbf{0.631} & \textbf{0.726}  & 0.117 & 0.248                  & \textbf{0.150} & \textbf{0.226}  \\ \hline
\end{tabular}

